Modeling and Trajectory Optimization for Standing Long Jumping of a Quadruped with A Preloaded Elastic Prismatic Spine

This paper presents a novel methodology to model and optimize trajectories of a quadrupedal robot with spinal compliance to improve standing jump performance compared to quadrupeds with a rigid spine. We introduce an elastic model for a prismatic robotic spine that is actively preloaded and mechanically lock-enabled at initial and maximum length, and develop a constrained trajectory optimization method to co-optimize the elastic parameters and motion trajectories toward enhanced jumping distance. Results reveal that a less stiff spring is likely to facilitate jumping performance not as a direct propelling source but as a means to unleash more motor power for propelling by trading-off overall energy efficiency. We also visualize the impact of spring coefficients on the overall optimization routine from energetic perspectives to identify the suitable parameter region.

==> Equations/CoT.tex <==
\begin{equation}
\boldsymbol{CoT}=
\frac{\boldsymbol{P}}{m g v_{ss}}
\end{equation}

==> Equations/Ellipsoidal_Trajectory.tex <==
\begin{equation}
\left[\begin{array}{l}{x} \\ {y}\end{array}\right]
=
\left[\begin{array}{l}{a\cos{\theta}} \\ {b\sin{\theta}}\end{array}\right],
0 \leq \theta < 2\pi \\
\end{equation}

%% \begin{equation}
%% \left[\begin{array}{l}{\Dot{x}} \\ {\Dot{y}}\end{array}\right]
%% =
%% \left[\begin{array}{l}{-a\Dot{\theta}\sin{\theta}} \\ {b\Dot{\theta}\cos{\theta}}\end{array}\right],
%% 0 \leq \theta < 2\pi \\
%% \end{equation}

where the polar angle $\theta$ is the phase of an oscillator, $a$ and $b$ correspond to the semi-major axis and semi-minor axis of an ellipse, respectively. To describe two half-ellipsoids that share the same semi-major axis, these parameters in our context are defined piece-wise as:

\begin{equation}
\begin{aligned}
a &= w/2 \\
b &= \left\{\begin{array}{ll}
{h_{\text{up}},} & {\text { if } 0 \leq \theta < \pi} \\ 
{h_{\text{down}},} & {\text { if } \pi \leq \theta < 2\pi}\end{array}\right.\\
\end{aligned}
\end{equation}

where $w$ is stride length, $h_{\text{up}}$ is up-amplitude, and $h_{\text{down}}$ is down-amplitude. Reference states $\boldsymbol{p}_{\text{ref}} = \left[ \alpha_{\text{ref}}, \beta_{\text{ref}}\right]^{\top}$ in the motors' configuration space are computed at 100 Hz based on foot states in Cartesian coordinates. The relation between them is

\begin{equation}
\left[\begin{array}{l}{x} \\ {y}\end{array}\right]
=
\left[\begin{array}{l}{L_{1} \sin{\alpha_{\text{ref}}} - L_{2} \sin{\beta_{\text{ref}}}} \\ 
{L_{1} \cos{\alpha_{\text{ref}}} + L_{2} \cos{\beta_{\text{ref}}}}\end{array}\right],
0 \leq \theta < 2\pi \\
\end{equation}

where $L_{1}$ and $L_{2}$ are the lengths of the upper and lower limbs.



==> Equations/Leg_Jacobian.tex <==
\begin{equation}
\boldsymbol{J}
=
\left[\begin{array}{ll}
{L_{1}\cos{\alpha}} & {-L_{2}\cos{\beta}} \\ 
{-L_{1}\sin{\alpha}} & {-L_{2}\sin{\beta}}
\end{array}\right]
\end{equation}

==> Equations/PD_Feedforward_Controller.tex <==
\begin{equation}
\boldsymbol{\tau}=
\left[ \boldsymbol{K}_{p} \left( \boldsymbol{p}_{\text{ref}} - \boldsymbol{p} \right)
+ \boldsymbol{K}_{d} \left( \Dot{\boldsymbol{p}}_{\text{ref}} -\Dot{\boldsymbol{p}}\right)\right] 
+ \boldsymbol{\tau}_{\text{ff}}
\end{equation}

where $\boldsymbol{K}_{p}$ and $\boldsymbol{K}_{d}$ are diagonal matrices for proportional and derivative gains. $\boldsymbol{p}_{\text{ref}}$ and $\Dot{\boldsymbol{p}}_{\text{ref}}$ are sent from a trajectory generator, and $\boldsymbol{p}$ and $\Dot{\boldsymbol{p}}$ are estimated on the leg controller. The feed-forward term $\boldsymbol{\tau}_{\text{ff}}$ is computed based on the dynamics of the spring-loaded virtual leg which can be modeled as

\begin{equation}
\begin{aligned}
\boldsymbol{\tau}_{\text{ff}}&=
\boldsymbol{J}^{\top} \boldsymbol{F}_{\text{spring}} \\
|\boldsymbol{F}_{\text{spring}}| &= k_{\text{spring}} (|\boldsymbol{p}| - l_{0})
\end{aligned}
\end{equation}

where $\boldsymbol{F}_{\text{spring}}$ is the desired ground contact force exerted by the virtual leg, $k_{\text{spring}}$ is the preset virtual spring constant, and $\boldsymbol{J}$ is the foot Jacobian.

==> IROS_Reviews.tex <==
% Comments to author (Associate Editor)
=====================================

Although the paper presents an interesting approach for
long jumps of quadruped robots, the reviewers expressed
some fundamental concerns especially when defining the
associated optimisation problem. The authors are strongly
encouraged to clarify these points prior to publication. 


% Reviewer 1 of IROS 2021 submission 2013

Comments to the author
======================

The paper focuses on analyzing a model for quadruped robots
that uses a compliant spine, and whether this could help in
improving standing long jump. The compliant spine is
represented by a prismatic joint with a preloaded spring,
which can be locked at min and max lengths via a motor.
The rationale is based on the fact that animals in nature
use their bodies to help their jumping, while many current
quadruped robots mostly rely on their strong leg actuation.
The model is a 5 links 2D model, and the assumption that
the legs are much lighter to the point of neglecting them
is made in order to simplify the dynamics, and a force
explicit elastic model based on Hooke's law is used to
describe the elasticity. The jumping motion is modeled as a
symmetric multiple-phase motion with pre-determined
timings, and the optimization aims at maximizing jumping
distance, while also optimizing for the resting length and
elastic constant. The results show that the compliant spine
can improve jumping distance by more than 20% with respect
to the rigid model.

The paper is overall well-written, with a proper
motivation, good rationale, and novelty. There are however
some points the authors should consider
clarifying/improving in order to enhance the quality of
their paper:
- To my understanding, the authors imposed the length of
the spine to be the same as the rigid model, is this "just"
to compare with the rigid model, or are there other reasons
to do so? I would have thought that otherwise this could
also be optimized for as well, with proper constraints.
- How were the dynamic parameters of the robot decided? The
parameters are shown in Table I, but not discussed. Are
these based on existing platforms? Are they chosen based on
rationale, e.g. about motors as the authors mention later
in the paper? 
- How was the timing of the phases chosen?
- The authors mention that two configurations have been
used: knee-backward and knee-forward, I did not fully
understand whether the authors have actually run
optimization with both configurations and observed
differences or just have decided for one (knee-forward)
based on literature? In this case, it would be somewhat
confusing that in Fig. 2 both configurations appear.
- Section IV.C should appear much earlier, as it directly
impacts the outcomes shown in section IV.B. Otherwise the
reading may be confusing at this point of the paper.
- In section IV.C the authors refer to the benefit
indicator as "B", this notation should appear also in Fig.
5.

Comments on the ICRA-21 Paper Attachment
========================================

I think the authors have well-summarized the main
weaknesses of their previous submission and have properly
explained how these have been addressed in the revised
version of the paper.

% Reviewer 3 of IROS 2021 submission 2013

Comments to the author
======================

The aim of the paper goes toward the direction of enhancing
robot capabilities by rethinking robot bodies with design
principle inspired by nature. 
The authors propose a quadruped with compliance spine by
introducing a spring-loaded prismatic joint. The prismatic
joint can be locked at predefined initial and final length,
thus a hybrid model is required to switch from rigid to
elastic behaviour.
The authors' contributions are:
- a simplified 2-D model of a quadruped with elastic
elements
- an offline trajectory optimization
- a co-design strategy for helping the designer in the
choice of spring characteristics

The topic studied is innovative and important, but there
are some issues that should be clarified:

1. The aim of the trajectory optimization is to maximize
the standing jump distance. However (8) minimizes "J" (a
function proportional to the take of velocity). Is it a
typo? 

2. The definition of the state "X" in eq.(8) is not
perfectly clear and should be clarified. 
What is it "t"? Is "t" part of the optimization problem? Is
"X" a high-level formulation to simply the notation?

3. Why are the spring parameters ($k_s$ and $l_{s,rest}$)
time-varying in the formulation of the constraints of the
compliant model?

4. The addition of a spring and a motor might cause an
increase of robot weight. I would suggest the author to do
some consideration about this aspect, and in case the
increase is relevant, they could add extra weight in the
hybrid model in order to do a  fair comparison with the
rigid model.

5. "As indicated in Fig. 2, we adopted two arrangements for
hind leg as knee-backward and knee-forward. [...]. Results
obtained herein, appear to suggest that knee-forward hind
legs are more likely to produce better solutions with less
computing time even though both arrangements should be
dynamically identical in principle."
I would suggest the authors to enforce their statement with
numbers and results to help the readers to quantitatively
understand the differences.

6. Section IV misses information on the implementation.
    - Which is time step Ts selected? 
    - Which is the torque limit value used in the
optimization problem? 
    - Which is the computational time for solving the
offline trajectory optimization?
    - How does the time system integration is implemented?
Which is integration technique adopted?


Comments on the ICRA-21 Paper Attachment
========================================

The authors clarified the concern raised about the MPC
formulation, they provided an additional set of results.
Moreover they fix the lack of literature review.
However, here are still some small inaccuracies in the
definition of the trajectory optimizati

==> Image Input/figure1.tex <==
\begin{figure}[!t]
	\vspace{6pt}
	\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{Figures/description_of_models.png}
	\vspace{0pt}
	\caption{\textbf{Sagittal Plane Models.} This figure shows 5-link model (left) and proposed hybrid model with lock-enabled springy prismatic spine (right), with purple fore legs, yellow hind legs, and blue torsos. General coordinates, posture descriptor, and control inputs are denoted.}
	\label{fig:models}
	\vspace{-16pt}
\end{figure}

==> Image Input/figure2.tex <==
\begin{figure}[!th]
	\vspace{6pt}
	\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{Figures/jump_phases_modes.png}
	\vspace{0pt}
	\caption{\textbf{Stand Jump Process and Time Schedule.} This figure shows that \textbf{(a)} a stand jump consists of double-contact $P_{dc}$, single-contact $P_{sc}$, and no-contact $P_{nc}$ phases before landing at $T_5$ for both models, switched by events as fore-foot-liftoff at $T_1$ and hind-foot-liftoff at $T_2$; \textbf{(b)} Takeoff happens during $T_0$ to $T_2$; \textbf{(c)} The proposed model (bottom) also experiences frozen mode $M_{fr}$ and springy mode $M_{sp}$, switched by events as spring-release at $T_3$ and spring-lock at $T_4$; \textbf{(d)} Hind legs can be arranged as knee-backward (top) or knee-forward (bottom).}
	\label{fig:jump_phases_modes}
	\vspace{-16pt}
\end{figure}

==> Image Input/figure3.tex <==
\begin{figure}[!t]
	\vspace{6pt}
	\centering
\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=\linewidth]{Figures/workflow.png}
	\vspace{0pt}
	\caption{\textbf{Modeling and Control Architecture.}}
	\label{fig:Workflow}
	\vspace{-16pt}
\end{figure}

==> Image Input/figure4.tex <==
\begin{figure}[!t]
	\vspace{6pt}
	\centering
        \includegraphics[trim={0.5cm 0cm 1cm 0.15cm},clip,width=\linewidth]{Figures/compliance_shaping_v6.eps}
	\vspace{0pt}
	\caption{\textbf{Compliance Property Shaping.} Elastic property results from shaping, including sample filtering and line fitting. Refined characteristics line is provided by nominal trajectory planner.}
	%as springy-mode samples (black dot), initial guess of elasticity relation (blue line), and refined spring characteristics (red line).
	\label{fig:compliance_shaping}
	\vspace{0pt}
\end{figure}



\iffalse
\begin{figure}[!t]
	\vspace{6pt}
	\centering
    \begin{subfigure}[t]{0.45\linewidth}	
        \centering
        \includegraphics[trim={1cm 0cm 1cm 0cm},clip,width=\linewidth]{Figures/compliance_shaping.png}
        \caption{}
	\end{subfigure}
	\quad
	\begin{subfigure}[t]{0.45\linewidth}
	    \centering
        \includegraphics[trim={1cm 0cm 1cm 0cm},clip,width=\linewidth]{Figures/spring_coeffs_vs_jump_dist_20percent.png}
        \caption{}
    \end{subfigure}
	\vspace{0pt}
	\caption{\textbf{Compliance Property Shaping and Sensitivity Analysis.} \textbf{(a)} is the compliance shaping results: springy-mode samples (black dot), initial guess of elasticity relation (blue line), and refined spring characteristics (red line). \textbf{(b)} shows the maximum jump distance with different spring properties. Both Graph use the same time schedule and initial posture as section \ref{subsect:stand_long_jump}.}
	\label{fig:compliance_shaping}
	\vspace{-16pt}
\end{figure}
\fi

==> Image Input/figure7.tex <==
\begin{figure}[!t]
	\vspace{6pt}
	\centering
\includegraphics[trim={0cm 0cm 0cm 0.5cm},clip,width=\linewidth]{Figures/spring_coeffs_vs_jump_dist_88samples_v2.eps}
	\vspace{0pt}
	\caption{\textbf{Impact of Elastic Characteristics.} Relation between elastic coefficients ($k_s$, $l_{s,rest}$) and jumping distance upper-bound $D_s$ for the hybrid model. The sign of $D_s$ is reverted to correspond to minimum cost. The planes represent rigid model's maximum jumping distance $D_r$ and its extensions, from top to bottom as $D_r$, $110\% D_r$, and $120\% D_r$.}
	\label{fig:spring_coeffs_vs_jump_dist}
	\vspace{-16pt}
\end{figure}

==> RandomThoughts.tex <==
% What are the major challenges
To advance performance upper-bound along certain partially unknown evolving pattern makes the problem many unknown parameters to identify, including spring constant, spring initial length, spring rest length, spring release time, and spring locking time. Under the context of nonlinear and non-convex optimization, random try-and-test for these parameters is more of art and can be quite time consuming. To face this challenge, we separate the parameter identification problem into 2 steps, each solved in a nonlinear MPC problem: firstly we try out time parameters with no assumption of spine internal force to identify a feasible set for time parameters; secondly, we conduct curve fitting upon force-displacement results within the spring mode (defined by T3 and T4) to get initial guess of spring parameters that are set for nonlinear MPC problem to minimize the final distance error (or maximize the final distance). 

% Why do not mimic kinematic data captured from real animals
Literature has shown some work to mimic animal motion on legged robots from kinematic data. While these work can reproduce lively motion, it is less likely to provide concrete insights on how to advance robot structure design that can extend maneuverability upper-bound. On the other hand, optimization methods provide a straightforward way to indicate object upper-bound, as here the maximum leap distance, by including the criterion in cost function.

% Leg structure
By excluding foot segment, articulated leg has two typical types, two-segment and three-segment (see cheetah-cub), both of which have been implemented in recent years. Mammalian animals features three-segment hind legs that propel them forward aggressively and can be approximated by pantograph leg design. Kinematic equivalence of this three-segment leg results in two arrangements of two-segment leg (need a fig here). Both hind leg arrangements were implemented and the folding-forward arrangement performs better in terms of solution feasibility in the optimization problem. One possible reason is that the folding-forward arrangement can exert larger GRF under the same actuator limitation (May need a fig to compare these two: same virtual leg length and attach angle 60, 90, 120, see Fx and Fz range).

% Possible explanation of no cat-like jump
Fore leg shoulder joint being rotational is a strong assumption.
The muscle-actuated scapula in mammalian animals allows for both rotation and translation, such feature may be critical to present a cat-like jump.

% Selection Matrix
Following previous work, we adopt 2-phase takeoff procedure (i.e., firstly fore foot lifts up, then rear foot lifts up) with a predefined time schedule. Thus the selection coefficients to indicate foot contact event are time-dependant.

% Trade-off between reducing nonlinearity in EoMs and constraintss
The revised EoMs attain more freedom to tune inputs and thus increase the chance to converge to a feasible or optimal solution. This modification also has a less explicit advantage for solver's numerical stability because it only requires inversion over generalized mass matrix $M$ which is constant diagonal matrix; on the other hand, EoMs from section \ref{subsec:full_dynamics} have to undertake inversion of time-variant matrices. Nevertheless, we admit that the modification applies more nonlinear inequality constraints to the optimization problem (see section X) but it is not observed to undermine the overall NLP solver performance during the implementation.

% Initial Guess of Spring parameters
Why we need to find the initial guess for the parameter values first? Because it is obscure to simply select values that may satisfy the system requirement. Because the non-convexity of the nonlinear mpc problem, a bad choice of initial values may lead to disappointing results. Thus we need a good guess that can at least partially reflect the system performance. Here we replace the spring force with an arbitrary force exerted from a massless linear actuator. Certain constraints are applied to confine the force-displacement pattern close to spring-like one and use the results for line fitting of initial spring parameter guess.

% Why enabling locking for spring
In the previous work, the spine have been modeled as spring or spring-damping systems to investigate gait stability. Video evidence of quadrupedal animals, especially leaping masters like Bobcats, indicates the stiffness change within their torso during amazing leap. Therefore, we use spring and rigid modes for the torso of different stiffness levels and regulate their transition through locking mechanism. 

% Observation of Bobcat stand jump
The rigid body model demonstrates a frog-like jump that presents a large body pitch angle (Cheetah3 shows it too) and the fore leg acts to tilt up the body. On the other hand, a Bobcat shows a more flat jumping posture when it uses the fore legs to direct the body both forward and upward while the hip is moving slower forward and squeezes the rear legs. Its torso becomes more rigid when the fore legs takeoff but the stiffness change is smooth.

% Question raised from the observation
The fact that Bobcats can leap several times of its body length with a elegant posture transition implies the cat-like leap a proper way to spring the body forward and increase the leap distance upper-bound. However,
what is the underlying rule of the cat-like leap? Is the spring model a good candidate?

% Initial Conditions
As one may expect, the initial posture can play an vital role in feasibility and optimality of the solution. Trying out values for all states and inputs randomly is not a well-organized way. Here we define the initial conditions according to Figure X as $\boldsymbol{p}_0 = \left[ x_0, z_0, \theta_0, \alpha_f, \alpha_r \right]$, where $\alpha_f$ and $\alpha_r$ are attacking angles of fore and rear virtual legs from hip to foot.

==> Tables/Physical_Property_of_Quadrupedal_Robot.tex <==
%[Table to show the common physical properties of state-of-the-art legged robots]\\
\begin{table}[!h]
\vspace{0pt}
    \caption{Physical Properties of Quadrupedal Robots}
    \vspace{-3pt}
    \label{table:improvement}
    \begin{center}
    \begin{tabularx}{\columnwidth}{|X|X|X|X|X|X|}
        \hline
        \textbf{Robot} & \textbf{Total DOF} & \textbf{Leg Length} & \textbf{Total Mass} & \textbf{Mass of Motors} & \textbf{Reduction Ratio} \\
         & \textbf{(Actuated DOF)} & \textbf{(m)} & \textbf{(kg)} & \textbf{($\%$)} & \\
        \hline
        CLL
        & $12(8 or 12)$ & $0.38$ & NA & NA & $3$ \\
        \hline
        Doggo
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\
        \hline
        MIT Mini Cheetah
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\ %TODO
        \hline
        MIT Cheetah 3
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\ %TODO
        \hline
        MIT Cheetah 2
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\ %TODO
        \hline
        Minitaur
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\ %TODO
        \hline
        ANYMAL
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\ %TODO
        \hline
        StarlETH
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\ %TODO
        \hline
        Cheetah Cub
        & $8(8)$ & $0.16$ & $4.8$ & $35$ & $3$ \\ %TODO
        \hline
    \end{tabularx}
    \end{center}
    \vspace{-8pt}
\end{table}

==> prop1.tex <==
%\begin{proposition}\label{lma2}
%Under the conditions i) of the original optimal steering problem~\cite{chen2016optimal1}, ii) $b_{1_{x},wall}=b_{1_{x},free}$ and $b_{1_{y},wall} \leqslant b_{1_{y},free}$ %for the diffusion coefficients,  and iii) $\sigma_{x,free}(0)=\sigma_{x,wall}(0)$ and $\sigma_{y,free}(0)=\sigma_{y,wall}(0)$, the control energy when interacting with obstacles to navigate through an aperture is less than the control energy to optimally steer the robotic agent directly to target as if there were no obstacles. %of the robot goes from the initial distribution to the final distribution with a finite interval. If the robot interacts with the environmental boundary by performing door entering behavior, the control energy of that robot is less than and equal to the optimal control energy without boundary. 
%\end{proposition} 
%\begin{proof}
Let $k_{x}(t)$ and $k_y(t)$ be as in the linear optimal steering in both free motion and wall-following. The initial distribution and end time stay the same too. When colliding with the wall, the control energy in the $x$ direction is
%
\begin{equation}\label{eq:cost}
\begin{aligned} 
J_{x,wall}=&\int\limits_{0}^{T_{i}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt+\int\limits_{T_{i}}^{T_{d}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt \\
& +\int\limits_{T_{d}}^{T}k^{2}_{x}(t)\sigma_{x,wall}(t)dt \enspace,
\end{aligned} 
\end{equation}
%
where $T_{i}$ and $T_{d}$ denote the time of impact and disengaging from the wall, respectively. 

We can split the control energy required to perform the same task as if there were no obstacles in three parts, according to switching times $T_{i}$ and $T_{d}$.  That is, $J_{x,free} = J_{1}(0\le t \le T_i) + J_{2}(T_i\le t \le T_d) + J_{3}(T_d\le t \le T)$. According to noise kinematics~\eqref{eq11} and due to the condition $\sigma_{x,free}(0)=\sigma_{x,wall}(0)$, then $\sigma_{x,wall}(t)=\sigma_{x,free}(t)$ $t\in [0, T_{i}]$. Hence $J_{1} = \int\limits_{0}^{T_{i}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt$.  Following the same rationale, and assuming that the processes are stationary~\cite{chen2016optimal1} so that we can time swift $J_{3}$ from $t=T_d$ to $t=0$, we get that $J_{3} = \int\limits_{T_{d}}^{T}k^{2}_{x}(t)\sigma_{x,wall}(t)dt$. 
%The Lyapunov differential equation is the same as \eqref{eq8} for the free motion mode. 
%
In wall-following mode the Lyapunov differential equation in $x$ direction is chosen to be 
%
\begin{equation}\label{eq14} %\tag{12a}
\dot{\sigma}_{x,wall}(t)=2b_{x}h_{x}(t)+b_{1_{x},wall}^{2}-Q(t)\enspace.
\end{equation}

$Q(t)$ is added to account for the wall-following effect on $\sigma_{x}(t)$. We consider $Q(t)\geqslant 0$ since the wall-following motion decreases the rate of diffusion over the $x$ direction~\cite{stager2016stochastic}. Therefore, we get $\sigma_{x,wall}(t) \leqslant \sigma_{x, free}(t)$. Then 
%
%\begin{equation}\label{eq12}
\begin{align*}
%J_{2_{x,ape}}& =
\int\limits_{T_{i}}^{T_{d}}k^{2}_{x}(t)\sigma_{x,wall}(t)dt&=\lim \limits_{n\to \infty}\sum \limits_{i=1}^{n} k _{x}^{2}(\xi_{i})\sigma_{x,wall}(\xi_{i})\Delta t \\
& \leqslant  \lim \limits_{n\to \infty}\sum \limits_{i=1}^{n} k _{x}^{2}(\xi_{i})\sigma_{x, free}(\xi_{i})\Delta t\\
&=\int\limits_{T_{i}}^{T_{d}}k^{2}_{x}(t)\sigma_{x, free}(t)dt 
= J_2
\end{align*}
%\end{equation}
%
with $\xi_{i} \in [t_{i}, t_{i+1})$. 
%
Thus, $J_{x,wall} \le J_{x,free}$. 

The same steps apply to the control energy along the $y$ direction. For wall-following when $t\in(T_{i},T_{d}]$, $b_{1_{y}, wall}^{2}\leqslant b_{1_{y},free}^{2}$ and based on the noise kinematics
%
% k^{2}_{x}(\xi)\int\limits_{0}^{T}\sigma_{x, wall}(t) \leqslant k^{2}_{x}(\xi)\int\limits_{0}^{T}\sigma_{x, free}(t)
%
\begin{equation}\label{eq15} %\tag{12b}
\dot{\sigma}_{y,wall}(t)=2b_{y}h_{y}(t)+b_{1_{y},wall}^{2}\enspace,
\end{equation}
%
we get $\sigma_{y,wall}(t) \leqslant \sigma_{y, free}(t)$ leading to 
%
%During the wall-following section $(T_{i},T_{d}]$ $b_{1_{y}, wall}^{2}\leqslant b_{1_{y},free}^{2}$, we get  $\sigma_{y, ape}^{col}(t) \leqslant \sigma_{y, free}(t)$. 
%
%that leads to $J_{y, wall}=\int\limits_{0}^{T}k^{2}_{y}(t)\sigma_{y, wall}(t)=k^{2}_{y}(\xi)\int\limits_{0}^{T}\sigma_{y, wall}(t) \leqslant k^{2}_{y}(\xi)\int\limits_{0}^{T}\sigma_{y, free}(t)$. 
$J_{y, wall} \leqslant J_{y, free}$. 
%
Since motions in the $x$ and $y$ directions are assumed independent from each other, $J_{wall}=J_{x,wall}+J_{y,wall} \le J_{x,free}+J_{y,free}=J_{free}$. %, which concludes the proof.
%\kkb{Combining the motion in both directions we deduce that $J_{2\ x,wall}+J_{2\ y, ape}^{col} \leqslant J_{2\ x, free}+J_{2\ y, free}$.  
%
%Similarly, since $\sigma_{x,ape}^{col}(T_{d}) \leqslant \sigma_{x,free}(T_{d})$ and  $\sigma_{y,ape}^{col}(T_{d}) \leqslant \sigma_{y,free}(T_{d})$, from \eqref{eq12}, the we can get the inequality holds in the disengaging period $(T_{d},T]$.  Hence we get $J_{3\ x, ape}^{col}+J_{3\ y, ape}^{col} \leqslant J_{3\ x, free}+J_{3\ y, free}$ . 
%We can prove that$J_{ape}^{col} \leqslant J_{free}$.}
%\end{proof}

As an immediate consequence, and by the triangle inequality on the system's stochastic process, we get $J_{wall} \le J_{free} \le J_{ncol}$, where $J_{ncol}$ denotes the control energy to steer through the aperture without collision.

%\begin{corollary}\label{col1}
%Piece-wise optimal steering through the aperture within the same time interval requires more energy than interacting with obstacles to navigate through the aperture.
%\end{corollary}
%\begin{proof}
%Let $J_{ncol}$ %=J'_1(0 \le t \le T_{ape}) + J'_2(T_{ape} \le t \le T)$ 
%denote the control energy to steer through the aperture without collision. %, with $T_{ape}$ being the time of passing through the aperture.
%By the triangle inequality on the system's stochastic process, and due to Proposition~\ref{lma2}, we get $J_{wall} \le J_{free} \le J_{ncol}$. % yields $||J_{free}|| \le ||J'_1|| + ||J'_2|| = ||J_{ncol}||$.  proposition~\ref{lma2}, it then follows that
%\kkb{It follows directly from Proposition 1, we get $J_{ape}^{col} \leqslant J_{free}$. Since the feasible set of piece-wise optimal steering  is the subset of optimal steering problem. Then it is easy to prove $J_{ape}^{col} \leqslant J_{free} \leqslant J_{ape}^{ncol}$.}
%\end{proof}
